Functional mesoscale organization of complex networks

The network density matrix (NDM) framework, enabling an information-theoretic and multiscale treatment of network flow, has been gaining momentum over the last decade. Benefiting from the counterparts of physical functions such as free energy and entropy, NDM's applications range from estimating how nodes influence network flows across scales the centrality of nodes at the local level to explaining the emergence of structural and functional order. Here, we introduce a generalized notion of the network internal energy $E_\tau$, where $\tau$ denotes a temporal hyperparameter allowing for multi-resolution analysis, showing how it measures the leakage of dynamical correlations from arbitrary partitions, where the minimally leaky subsystems have minimal $E_\tau$. Moreover, we analytically demonstrate that $E_\tau$ reduces to the well-known modularity function at the smallest temporal scale $\tau = 0$. We investigate this peculiar resemblance by comparing the communities minimizing $E_\tau$, with those detected by widely used methods like multiscale modularity and Markov stability. Our work provides a detailed analytical and computational picture of network generalized internal energy, and explores its effectiveness in detecting communities in synthetic and empirical networks within a unifying framework.

==> data/flights-silhouette.tex <==

\pgfplotstableread[
col sep=comma,
header=true,
]{
name,rank,clean_method,method,inertia,tau_ix,sil
flightsWorld,1,RWTen,RW-10,10,12,0.13879
flightsWorld,2,RWOne,RW-1,1,12,0.13846
flightsWorld,3,RWFour,RW-4,4,12,0.13771
flightsWorld,4,RWFive,RW-5,5,12,0.13045
flightsWorld,5,RWThree,RW-3,3,12,0.12983
flightsWorld,6,RWFiveHundred,RW-500,500,10,0.12428
flightsWorld,7,RWFifty,RW-50,50,12,0.12167
flightsWorld,8,RWTwenty,RW-20,20,17,0.12068
flightsWorld,9,RWOneHundred,RW-100,100,12,0.11989
flightsWorld,10,RWFiveThousand,RW-5000,5000,12,0.11852
flightsWorld,11,RWTwo,RW-2,2,12,0.1181
flightsWorld,12,RW,RW,0,13,0.10615
flightsWorld,13,RWOneThousand,RW-1000,1000,10,0.10263
% flightsWorld,14,DiffFive,Diff-5,5,2,0.085638
% flightsWorld,15,DiffFour,Diff-4,4,2,0.085403
flightsWorld,16,MarkovRW,Markov-RW,0,14,0.071068
% flightsWorld,17,DiffThree,Diff-3,3,1,0.068138
% flightsWorld,18,DiffOne,Diff-1,1,15,0.067661
% flightsWorld,19,DiffTwo,Diff-2,2,15,0.067145
% flightsWorld,20,DiffTen,Diff-10,10,15,0.066756
flightsWorld,21,MultiLouvain,MultiLouvain,0,8,0.048224
% flightsWorld,22,DiffOneThousand,Diff-1000,1000,15,0.047395
% flightsWorld,23,DiffOneHundred,Diff-100,100,15,0.046071
% flightsWorld,24,DiffTwenty,Diff-20,20,15,0.044891
% flightsWorld,25,DiffFiveHundred,Diff-500,500,15,0.032697
% flightsWorld,26,Diff,Diff,0,14,0.029887
% flightsWorld,27,DiffFifty,Diff-50,50,15,0.024864
% flightsWorld,28,DiffFiveThousand,Diff-5000,5000,15,0.02364
flightsWorld,29,MarkovDiff,Markov-Diff,0,1,0
}{\FlightsWorldSilhouette}


%%% weighted sil
\pgfplotstableread[col sep=comma]{
name,rank,clean_method,method,inertia,tau_ix,weighted_sil
flightsWorld,1,RWTen,RW-10,10,12,0.14552
flightsWorld,2,RWFour,RW-4,4,12,0.14225
flightsWorld,3,RWFive,RW-5,5,12,0.13631
flightsWorld,4,RWOne,RW-1,1,12,0.12679
flightsWorld,5,RWFifty,RW-50,50,12,0.11802
flightsWorld,6,RWThree,RW-3,3,12,0.1173
flightsWorld,7,RWFiveThousand,RW-5000,5000,12,0.11649
flightsWorld,8,RWTwenty,RW-20,20,17,0.11621
flightsWorld,9,RWFiveHundred,RW-500,500,12,0.11408
flightsWorld,10,RWOneHundred,RW-100,100,12,0.11407
flightsWorld,11,RWTwo,RW-2,2,12,0.087927
flightsWorld,12,RW,RW,0,13,0.078632
flightsWorld,13,RWOneThousand,RW-1000,1000,10,0.065944
% flightsWorld,14,DiffFive,Diff-5,5,2,0.064871
% flightsWorld,15,DiffFour,Diff-4,4,2,0.055316
% flightsWorld,16,DiffThree,Diff-3,3,1,0.053996
flightsWorld,17,MarkovRW,Markov-RW,0,10,0.048287
% flightsWorld,18,DiffOne,Diff-1,1,15,0.014846
% flightsWorld,19,DiffTen,Diff-10,10,15,0.014599
% flightsWorld,20,DiffTwo,Diff-2,2,15,0.014502
flightsWorld,21,MultiLouvain,MultiLouvain,0,8,0.012682
% flightsWorld,22,DiffOneThousand,Diff-1000,1000,15,-0.0076407
% flightsWorld,23,DiffOneHundred,Diff-100,100,15,-0.009327
% flightsWorld,24,DiffTwenty,Diff-20,20,15,-0.010234
% flightsWorld,25,DiffFifty,Diff-50,50,1,-0.011673
% flightsWorld,26,DiffFiveHundred,Diff-500,500,15,-0.026759
% flightsWorld,27,Diff,Diff,0,14,-0.031098
% flightsWorld,28,DiffFiveThousand,Diff-5000,5000,1,-0.033264
flightsWorld,29,MarkovDiff,Markov-Diff,0,1,0
}{\FlightsWorldSilhouetteWt}


==> data/inertia-heatmap-data.tex <==
\pgfplotstableread[ignore chars={"}]{
    inertia mu EC EC_improv method avg_k family
    0 0.05 1 nan RW 10 LFROneK
    0 0.1 0.84 0 RW 10 LFROneK
    0 0.2 0.747 0 RW 10 LFROneK
    0 0.4 0.591 0 RW 10 LFROneK
    0 0.5 0.4334 0 RW 10 LFROneK
    0 0.6 0.1719 0 RW 10 LFROneK
    1 0.05 1 nan RW 10 LFROneK
    1 0.1 0.9164 0.090952 RW 10 LFROneK
    1 0.2 0.8972 0.20107 RW 10 LFROneK
    1 0.4 0.7966 0.34788 RW 10 LFROneK
    1 0.5 0.6509 0.50185 RW 10 LFROneK
    1 0.6 0.204 0.18674 RW 10 LFROneK
    2 0.05 1 nan RW 10 LFROneK
    2 0.1 0.9861 0.17393 RW 10 LFROneK
    2 0.2 0.9771 0.30803 RW 10 LFROneK
    2 0.4 0.8722 0.4758 RW 10 LFROneK
    2 0.5 0.6471 0.49308 RW 10 LFROneK
    2 0.6 0.2253 0.31065 RW 10 LFROneK
    3 0.05 1 nan RW 10 LFROneK
    3 0.1 1 0.19048 RW 10 LFROneK
    3 0.2 1 0.33869 RW 10 LFROneK
    3 0.4 0.8738 0.47851 RW 10 LFROneK
    3 0.5 0.685 0.58053 RW 10 LFROneK
    3 0.6 0.2334 0.35777 RW 10 LFROneK
    4 0.05 1 nan RW 10 LFROneK
    4 0.1 1 0.19048 RW 10 LFROneK
    4 0.2 0.9971 0.33481 RW 10 LFROneK
    4 0.4 0.8962 0.51641 RW 10 LFROneK
    4 0.5 0.6565 0.51477 RW 10 LFROneK
    4 0.6 0.2388 0.38918 RW 10 LFROneK
    5 0.05 1 nan RW 10 LFROneK
    5 0.1 1 0.19048 RW 10 LFROneK
    5 0.2 0.9891 0.3241 RW 10 LFROneK
    5 0.4 0.8779 0.48545 RW 10 LFROneK
    5 0.5 0.6506 0.50115 RW 10 LFROneK
    5 0.6 0.2374 0.38104 RW 10 LFROneK
    10 0.05 1 nan RW 10 LFROneK
    10 0.1 0.9861 0.17393 RW 10 LFROneK
    10 0.2 0.9971 0.33481 RW 10 LFROneK
    10 0.4 0.8923 0.50981 RW 10 LFROneK
    10 0.5 0.6519 0.50415 RW 10 LFROneK
    10 0.6 0.2323 0.35137 RW 10 LFROneK
    20 0.05 1 nan RW 10 LFROneK
    20 0.1 1 0.19048 RW 10 LFROneK
    20 0.2 0.9891 0.3241 RW 10 LFROneK
    20 0.4 0.8727 0.47665 RW 10 LFROneK
    20 0.5 0.6574 0.51684 RW 10 LFROneK
    20 0.6 0.2302 0.33915 RW 10 LFROneK
    50 0.05 1 nan RW 10 LFROneK
    50 0.1 1 0.19048 RW 10 LFROneK
    50 0.2 1 0.33869 RW 10 LFROneK
    50 0.4 0.8873 0.50135 RW 10 LFROneK
    50 0.5 0.6673 0.53969 RW 10 LFROneK
    50 0.6 0.2394 0.39267 RW 10 LFROneK
    100 0.05 1 nan RW 10 LFROneK
    100 0.1 1 0.19048 RW 10 LFROneK
    100 0.2 1 0.33869 RW 10 LFROneK
    100 0.4 0.8857 0.49865 RW 10 LFROneK
    100 0.5 0.653 0.50669 RW 10 LFROneK
    100 0.6 0.2387 0.3886 RW 10 LFROneK
    200 0.05 1 nan RW 10 LFROneK
    200 0.1 1 0.19048 RW 10 LFROneK
    200 0.2 1 0.33869 RW 10 LFROneK
    200 0.4 0.8841 0.49594 RW 10 LFROneK
    200 0.5 0.6571 0.51615 RW 10 LFROneK
    200 0.6 0.2363 0.37464 RW 10 LFROneK
    500 0.05 1 nan RW 10 LFROneK
    500 0.1 1 0.19048 RW 10 LFROneK
    500 0.2 1 0.33869 RW 10 LFROneK
    500 0.4 0.8804 0.48968 RW 10 LFROneK
    500 0.5 0.6431 0.48385 RW 10 LFROneK
    500 0.6 0.2345 0.36417 RW 10 LFROneK
    750 0.05 1 nan RW 10 LFROneK
    750 0.1 1 0.19048 RW 10 LFROneK
    750 0.2 1 0.33869 RW 10 LFROneK
    750 0.4 0.8871 0.50102 RW 10 LFROneK
    750 0.5 0.6757 0.55907 RW 10 LFROneK
    750 0.6 0.2328 0.35428 RW 10 LFROneK
    1000 0.05 1 nan RW 10 LFROneK
    1000 0.1 1 0.19048 RW 10 LFROneK
    1000 0.2 1 0.33869 RW 10 LFROneK
    1000 0.4 0.8858 0.49882 RW 10 LFROneK
    1000 0.5 0.6475 0.494 RW 10 LFROneK
    1000 0.6 0.2292 0.33333 RW 10 LFROneK
    2000 0.05 1 nan RW 10 LFROneK
    2000 0.1 1 0.19048 RW 10 LFROneK
    2000 0.2 1 0.33869 RW 10 LFROneK
    2000 0.4 0.8873 0.50135 RW 10 LFROneK
    2000 0.5 0.6442 0.48639 RW 10 LFROneK
    2000 0.6 0.235 0.36707 RW 10 LFROneK
    5000 0.05 1 nan RW 10 LFROneK
    5000 0.1 1 0.19048 RW 10 LFROneK
    5000 0.2 1 0.33869 RW 10 LFROneK
    5000 0.4 0.8855 0.49831 RW 10 LFROneK
    5000 0.5 0.6275 0.44785 RW 10 LFROneK
    5000 0.6 0.2268 0.31937 RW 10 LFROneK
}{\LFROneKkTENmethRWEC}

%%%%%%%%%%%%%%%%%

\pgfplotstableread[ignore chars={"}]{
    inertia mu EC EC_improv method avg_k family
    0 0.05 1 nan RW 15 LFROneK
    0 0.1 0.8533 0 RW 15 LFROneK
    0 0.2 0.7972 0 RW 15 LFROneK
    0 0.4 0.6867 0 RW 15 LFROneK
    0 0.5 0.5865 0 RW 15 LFROneK
    0 0.6 0.4703 0 RW 15 LFROneK
    1 0.05 1 nan RW 15 LFROneK
    1 0.1 0.9795 0.1479 RW 15 LFROneK
    1 0.2 0.9552 0.19819 RW 15 LFROneK
    1 0.4 0.9138 0.33071 RW 15 LFROneK
    1 0.5 0.9147 0.55959 RW 15 LFROneK
    1 0.6 0.8232 0.75037 RW 15 LFROneK
    2 0.05 1 nan RW 15 LFROneK
    2 0.1 1 0.17192 RW 15 LFROneK
    2 0.2 0.989 0.24059 RW 15 LFROneK
    2 0.4 1 0.45624 RW 15 LFROneK
    2 0.5 0.9625 0.64109 RW 15 LFROneK
    2 0.6 0.872 0.85414 RW 15 LFROneK
    3 0.05 1 nan RW 15 LFROneK
    3 0.1 1 0.17192 RW 15 LFROneK
    3 0.2 1 0.25439 RW 15 LFROneK
    3 0.4 0.9971 0.45202 RW 15 LFROneK
    3 0.5 0.9914 0.69037 RW 15 LFROneK
    3 0.6 0.8573 0.82288 RW 15 LFROneK
    4 0.05 1 nan RW 15 LFROneK
    4 0.1 1 0.17192 RW 15 LFROneK
    4 0.2 1 0.25439 RW 15 LFROneK
    4 0.4 1 0.45624 RW 15 LFROneK
    4 0.5 0.9818 0.674 RW 15 LFROneK
    4 0.6 0.8588 0.82607 RW 15 LFROneK
    5 0.05 1 nan RW 15 LFROneK
    5 0.1 1 0.17192 RW 15 LFROneK
    5 0.2 1 0.25439 RW 15 LFROneK
    5 0.4 1 0.45624 RW 15 LFROneK
    5 0.5 0.9943 0.69531 RW 15 LFROneK
    5 0.6 0.8859 0.88369 RW 15 LFROneK
    10 0.05 1 nan RW 15 LFROneK
    10 0.1 1 0.17192 RW 15 LFROneK
    10 0.2 0.9971 0.25075 RW 15 LFROneK
    10 0.4 1 0.45624 RW 15 LFROneK
    10 0.5 0.9723 0.6578 RW 15 LFROneK
    10 0.6 0.8671 0.84372 RW 15 LFROneK
    20 0.05 1 nan RW 15 LFROneK
    20 0.1 1 0.17192 RW 15 LFROneK
    20 0.2 1 0.25439 RW 15 LFROneK
    20 0.4 1 0.45624 RW 15 LFROneK
    20 0.5 0.9859 0.68099 RW 15 LFROneK
    20 0.6 0.8655 0.84031 RW 15 LFROneK
    50 0.05 1 nan RW 15 LFROneK
    50 0.1 1 0.17192 RW 15 LFROneK
    50 0.2 1 0.25439 RW 15 LFROneK
    50 0.4 1 0.45624 RW 15 LFROneK
    50 0.5 0.9943 0.69531 RW 15 LFROneK
    50 0.6 0.8374 0.78057 RW 15 LFROneK
    100 0.05 1 nan RW 15 LFROneK
    100 0.1 1 0.17192 RW 15 LFROneK
    100 0.2 1 0.25439 RW 15 LFROneK
    100 0.4 1 0.45624 RW 15 LFROneK
    100 0.5 0.9914 0.69037 RW 15 LFROneK
    100 0.6 0.8434 0.79332 RW 15 LFROneK
    200 0.05 1 nan RW 15 LFROneK
    200 0.1 1 0.17192 RW 15 LFROneK
    200 0.2 1 0.25439 RW 15 LFROneK
    200 0.4 1 0.45624 RW 15 LFROneK
    200 0.5 0.9914 0.69037 RW 15 LFROneK
    200 0.6 0.8425 0.79141 RW 15 LFROneK
    500 0.05 1 nan RW 15 LFROneK
    500 0.1 1 0.17192 RW 15 LFROneK
    500 0.2 1 0.25439 RW 15 LFROneK
    500 0.4 0.9971 0.45202 RW 15 LFROneK
    500 0.5 0.9914 0.69037 RW 15 LFROneK
    500 0.6 0.838 0.78184 RW 15 LFROneK
    750 0.05 1 nan RW 15 LFROneK
    750 0.1 1 0.17192 RW 15 LFROneK
    750 0.2 1 0.25439 RW 15 LFROneK
    750 0.4 0.9971 0.45202 RW 15 LFROneK
    750 0.5 0.9914 0.69037 RW 15 LFROneK
    750 0.6 0.8416 0.7895 RW 15 LFROneK
    1000 0.05 1 nan RW 15 LFROneK
    1000 0.1 1 0.17192 RW 15 LFROneK
    1000 0.2 1 0.25439 RW 15 LFROneK
    1000 0.4 0.9971 0.45202 RW 15 LFROneK
    1000 0.5 0.9914 0.69037 RW 15 LFROneK
    1000 0.6 0.8401 0.78631 RW 15 LFROneK
    2000 0.05 1 nan RW 15 LFROneK
    2000 0.1 1 0.17192 RW 15 LFROneK
    2000 0.2 1 0.25439 RW 15 LFROneK
    2000 0.4 0.9971 0.45202 RW 15 LFROneK
    2000 0.5 0.9886 0.68559 RW 15 LFROneK
    2000 0.6 0.8483 0.80374 RW 15 LFROneK
    5000 0.05 1 nan RW 15 LFROneK
    5000 0.1 1 0.17192 RW 15 LFROneK
    5000 0.2 1 0.25439 RW 15 LFROneK
    5000 0.4 0.9971 0.45202 RW 15 LFROneK
    5000 0.5 0.9914 0.69037 RW 15 LFROneK
    5000 0.6 0.855 0.81799 RW 15 LFROneK
}{\LFROneKkFIFTEENmethRWEC}

%%%%%%%%%%%%%%%%%

\pgfplotstableread[ignore chars={"}]{
    inertia mu EC EC_improv method avg_k family
    0 0.05 1 nan RW 20 LFROneK
    0 0.1 0.854 0 RW 20 LFROneK
    0 0.2 0.7797 0 RW 20 LFROneK
    0 0.4 0.6837 0 RW 20 LFROneK
    0 0.5 0.6741 0 RW 20 LFROneK
    0 0.6 0.5618 0 RW 20 LFROneK
    1 0.05 1 nan RW 20 LFROneK
    1 0.1 0.9881 0.15703 RW 20 LFROneK
    1 0.2 0.9632 0.23535 RW 20 LFROneK
    1 0.4 0.9304 0.36083 RW 20 LFROneK
    1 0.5 0.9183 0.36226 RW 20 LFROneK
    1 0.6 0.8938 0.59096 RW 20 LFROneK
    2 0.05 1 nan RW 20 LFROneK
    2 0.1 1 0.17096 RW 20 LFROneK
    2 0.2 1 0.28254 RW 20 LFROneK
    2 0.4 1 0.46263 RW 20 LFROneK
    2 0.5 1 0.48346 RW 20 LFROneK
    2 0.6 1 0.77999 RW 20 LFROneK
    3 0.05 1 nan RW 20 LFROneK
    3 0.1 1 0.17096 RW 20 LFROneK
    3 0.2 1 0.28254 RW 20 LFROneK
    3 0.4 1 0.46263 RW 20 LFROneK
    3 0.5 1 0.48346 RW 20 LFROneK
    3 0.6 0.9971 0.77483 RW 20 LFROneK
    4 0.05 1 nan RW 20 LFROneK
    4 0.1 1 0.17096 RW 20 LFROneK
    4 0.2 1 0.28254 RW 20 LFROneK
    4 0.4 1 0.46263 RW 20 LFROneK
    4 0.5 1 0.48346 RW 20 LFROneK
    4 0.6 0.9971 0.77483 RW 20 LFROneK
    5 0.05 1 nan RW 20 LFROneK
    5 0.1 1 0.17096 RW 20 LFROneK
    5 0.2 1 0.28254 RW 20 LFROneK
    5 0.4 1 0.46263 RW 20 LFROneK
    5 0.5 1 0.48346 RW 20 LFROneK
    5 0.6 0.9971 0.77483 RW 20 LFROneK
    10 0.05 1 nan RW 20 LFROneK
    10 0.1 1 0.17096 RW 20 LFROneK
    10 0.2 1 0.28254 RW 20 LFROneK
    10 0.4 1 0.46263 RW 20 LFROneK
    10 0.5 1 0.48346 RW 20 LFROneK
    10 0.6 0.9971 0.77483 RW 20 LFROneK
    20 0.05 1 nan RW 20 LFROneK
    20 0.1 1 0.17096 RW 20 LFROneK
    20 0.2 1 0.28254 RW 20 LFROneK
    20 0.4 1 0.46263 RW 20 LFROneK
    20 0.5 1 0.48346 RW 20 LFROneK
    20 0.6 0.9971 0.77483 RW 20 LFROneK
    50 0.05 1 nan RW 20 LFROneK
    50 0.1 1 0.17096 RW 20 LFROneK
    50 0.2 1 0.28254 RW 20 LFROneK
    50 0.4 1 0.46263 RW 20 LFROneK
    50 0.5 1 0.48346 RW 20 LFROneK
    50 0.6 0.9971 0.77483 RW 20 LFROneK
    100 0.05 1 nan RW 20 LFROneK
    100 0.1 1 0.17096 RW 20 LFROneK
    100 0.2 1 0.28254 RW 20 LFROneK
    100 0.4 1 0.46263 RW 20 LFROneK
    100 0.5 1 0.48346 RW 20 LFROneK
    100 0.6 0.9971 0.77483 RW 20 LFROneK
    200 0.05 1 nan RW 20 LFROneK
    200 0.1 1 0.17096 RW 20 LFROneK
    200 0.2 1 0.28254 RW 20 LFROneK
    200 0.4 1 0.46263 RW 20 LFROneK
    200 0.5 1 0.48346 RW 20 LFROneK
    200 0.6 0.9971 0.77483 RW 20 LFROneK
    500 0.05 1 nan RW 20 LFROneK
    500 0.1 1 0.17096 RW 20 LFROneK
    500 0.2 1 0.28254 RW 20 LFROneK
    500 0.4 1 0.46263 RW 20 LFROneK
    500 0.5 1 0.48346 RW 20 LFROneK
    500 0.6 0.9971 0.77483 RW 20 LFROneK
    750 0.05 1 nan RW 20 LFROneK
    750 0.1 1 0.17096 RW 20 LFROneK
    750 0.2 1 0.28254 RW 20 LFROneK
    750 0.4 1 0.46263 RW 20 LFROneK
    750 0.5 1 0.48346 RW 20 LFROneK
    750 0.6 0.9971 0.77483 RW 20 LFROneK
    1000 0.05 1 nan RW 20 LFROneK
    1000 0.1 1 0.17096 RW 20 LFROneK
    1000 0.2 1 0.28254 RW 20 LFROneK
    1000 0.4 1 0.46263 RW 20 LFROneK
    1000 0.5 1 0.48346 RW 20 LFROneK
    1000 0.6 0.9971 0.77483 RW 20 LFROneK
    2000 0.05 1 nan RW 20 LFROneK
    2000 0.1 1 0.17096 RW 20 LFROneK
    2000 0.2 1 0.28254 RW 20 LFROneK
    2000 0.4 1 0.46263 RW 20 LFROneK
    2000 0.5 1 0.48346 RW 20 LFROneK
    2000 0.6 0.9971 0.77483 RW 20 LFROneK
    5000 0.05 1 nan RW 20 LFROneK
    5000 0.1 1 0.17096 RW 20 LFROneK
    5000 0.2 1 0.28254 RW 20 LFROneK
    5000 0.4 1 0.46263 RW 20 LFROneK
    5000 0.5 1 0.48346 RW 20 LFROneK
    5000 0.6 0.9971 0.77483 RW 20 LFROneK
}{\LFROneKkTWENTYmethRWEC}

%%%%%%%%%%%%%%%%%


==> preamble.tex <==
\RequirePackage[sort&compress]{natbib}

%\usepackage{listings}
%\usepackage{graphicx}
%\usepackage{epstopdf}
%\usepackage{multirow}
\usepackage{color}
\usepackage{xspace}
%\usepackage{amssymb,amsfonts,amsmath}
%\usepackage[english]{babel}
%\usepackage{float}
%
%

\usepackage{amssymb,amsfonts,amsmath}
\usepackage{bm}
\usepackage[pdftex]{graphicx}
\usepackage[all]{nowidow}
\usepackage[dvipsnames]{xcolor}
%\usepackage{setspace}
\usepackage{comment}

%after xcolor
\usepackage[colorlinks = true,
            linkcolor = blue,
            urlcolor  = blue,
            citecolor = blue,
            anchorcolor = blue]{hyperref}
\newcommand{\changeurlcolor}[1]{\hypersetup{urlcolor=#1}} 

\usepackage{dcolumn}% Align table columns on decimal point
\usepackage{bm}% bold math
%\usepackage{hyperref}% add hypertext capabilities
%\usepackage[mathlines]{lineno}% Enable numbering of text and display math
%\linenumbers\relax % Commence numbering lines

%\usepackage[showframe,%Uncomment any one of the following lines to test 
%%scale=0.7, marginratio={1:1, 2:3}, ignoreall,% default settings
%%text={7in,10in},centering,
%%margin=1.5in,
%%total={6.5in,8.75in}, top=1.2in, left=0.9in, includefoot,
%%height=10in,a5paper,hmargin={3cm,0.8in},
%]{geometry}


%\usepackage{subcaption}

%%%%%%%%%%%%%%%%%%
%PERSONAL MACRO
%%%%%%%%%%%%%%%%%%

\newcommand{\lto}[1]{\longrightarrow#1}
\newcommand{\rto}[1]{\longleftarrow#1}
\newcommand{\imply}[1]{\Longrightarrow#1}
\renewcommand{\(}{\left(}
\renewcommand{\)}{\right)}
\renewcommand{\[}{\left[}
\renewcommand{\]}{\right]}
\newcommand{\Eq}[1]{Eq.\,(\ref{#1})}
\newcommand{\Fig}[1]{Fig.\,\ref{#1}}
\newcommand{\tr}[1]{\text{Tr}\(#1\)}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\braket}[2]{\langle#1|#2\rangle}
\newcommand{\operator}[1]{{\mathbf{#1}}}

\newcommand{\eg}{\textit{e.g.}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\viz}{\textit{viz.}}
% satyaki macros
\renewcommand{\H}{\operator{H}}
\newcommand{\D}{\operator{D}}
\newcommand{\I}{\operator{I}}
\newcommand{\A}{\operator{A}}
\newcommand{\G}{\mathcal{G}_\tau}
\usepackage{multirow}

\newcommand{\ER}{Erd\"{o}s-R\'{e}nyi\xspace}

\newcommand{\arsham}[1]{{\color{red} Arsham: #1}}
\newcommand{\satyaki}[1]{{\color{teal} Satyaki: #1}}
\newcommand{\manlio}[1]{{\color{blue} Manlio: #1}}




%for non-pnas
\newcommand{\heading}[1]{{\vspace{0.25truecm}\noindent\textbf{#1.}}}
%for pnas
%\newcommand{\heading}[1]{\vspace{0.25truecm}\subsection{#1}}

\definecolor{RoyalBlue}{HTML}{4169e1}
\definecolor{ForestGreen}{HTML}{228b22}

\usepackage{setspace}
\usepackage{subfigure}
\usepackage{comment}

%for todos
\usepackage{todonotes}

\usepackage{tcolorbox}
\definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
\definecolor{alizarin}{rgb}{0.82, 0.1, 0.26}

\newcommand{\mdd}[1]{\textcolor{airforceblue}{#1}}
\newcommand{\notes}[1]{\begin{tcolorbox} Note: #1\end{tcolorbox}}
\newcommand{\rev}[1]{\textcolor{alizarin}#1}

%% PGFPLOTS stuff 
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usetikzlibrary{pgfplots.groupplots,arrows,automata,positioning,shapes.multipart,positioning,arrows,calc,backgrounds,fit,shapes,shapes.geometric}
\usepgfplotslibrary{dateplot,fillbetween,colormaps,colorbrewer}
% \selectcolormodel{cmyk}
\pgfplotsset{compat=1.18, lua backend=true}
% \usepackage{filecontents}
\usepackage[group-separator={,},group-minimum-digits=4]{siunitx}



\pgfplotsset{
  jitter/.style={
      y filter/.code={\pgfmathparse{\pgfmathresult+rnd*#1}}
  },
  jitter/.default=0.05
}
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}   %% some additional layers for demo
%%one bar symbol in pgfplot legend

\tikzstyle{every picture}+=[font=\sffamily] 
\pgfplotsset{every axis/.append style={
  font=\sffamily,
  label style={font=\sffamily\normalsize},
  title style={text depth=0.5ex,font=\sffamily\normalsize},
  tick label style={font=\sffamily\footnotesize, 
      /pgf/number format/assume math mode=true},  % for sans serif tick labels
  xtick align = center, 
  ylabel near ticks,
  y label style={font=\sffamily\normalsize},
  xlabel near ticks,
  x label style={font=\sffamily\normalsize},
  legend cell align={left},
  legend style={draw=none, font=\sffamily\small},
  },
  legend image code/.code={
  \draw[mark repeat=2,mark phase=2]
      plot coordinates {
      (0cm,0cm)
      (0.15cm,0cm)        %% default is (0.3cm,0cm)
      (0.3cm,0cm)         %% default is (0.6cm,0cm)
      };%
  },
  boxplot/hide outliers/.code={
    \def\pgfplotsplothandlerboxplot@outlier{}%
  }
}
  \pgfplotsset{
    jitter/.style={
        x filter/.code={\pgfmathparse{\pgfmathresult+(rnd-.5)*#1}}
    },
    jitter/.default=0.1
}


\usepackage[eulergreek]{sansmath}
\pgfplotsset{
  tick label style = {font=\sansmath\sffamily},
  every axis label = {font=\sansmath\sffamily},
  legend style = {font=\sansmath\sffamily},
  label style = {font=\sansmath\sffamily},
  title style = {font=\sansmath\sffamily}
}
\tikzset{every picture/.style={/utils/exec={\sffamily}}}


\pgfmathdeclarefunction{lg10}{1}{%
    \pgfmathparse{ln(#1)/ln(10)}%
}
\pgfplotscolorbarCMYKworkaroundfalse

%%% templates for different values of mu
\tikzstyle{mu5} = [
    smooth,
    thick,
    GnBu-D,
    mark=*, 
    mark options={thin, draw=GnBu-D!60!black, fill=GnBu-D!20, scale=0.5},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2, 
]

\tikzstyle{mu5_err} = [
    fill=GnBu-D!50,
    fill opacity=0.5,
]


\tikzstyle{mu10} = [
    smooth, 
    GnBu-F!95!black,
    mark=x, 
    % mark options={fill=Pastel-H},%, point meta=explicit symbolic, text=black,
    mark options={draw=GnBu-F!60!black, fill=GnBu-F!20, scale=0.80},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2,  
]

\tikzstyle{mu10_err} = [
    fill=GnBu-F!50,
    fill opacity=0.4,
]

\tikzstyle{mu20} = [
    smooth, 
    GnBu-H,
    mark=diamond, 
    % mark options={fill=Pastel-H},%, point meta=explicit symbolic, text=black,
    mark options={thin, draw=GnBu-H!80!black, scale=0.70},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2, 
]

\tikzstyle{mu20_err} = [
    fill=GnBu-H!50,
    fill opacity=0.5,
]


\tikzstyle{mu40} = [
    smooth, 
    GnBu-J,
    mark=star, 
    % mark options={fill=Pastel-H},%, point meta=explicit symbolic, text=black,
    mark options={draw=GnBu-J!70!black, fill=GnBu-J!20, scale=0.75},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2, 
]

\tikzstyle{mu40_err} = [
    fill=GnBu-J!50,
    fill opacity=0.5,
]

\tikzstyle{mu50} = [
    smooth, 
    GnBu-L,
    mark=square*, 
    % mark options={fill=Pastel-H},%, point meta=explicit symbolic, text=black,
    mark options={thin, draw=GnBu-L!80!black, fill=GnBu-L!50, scale=0.5},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2, 
]

\tikzstyle{mu50_err} = [
    fill=GnBu-L!50,
    fill opacity=0.5,
]

\tikzstyle{mu60} = [
    smooth, 
    GnBu-M,
    mark=oplus, 
    % mark options={fill=Pastel-H},%, point meta=explicit symbolic, text=black,
    mark options={thin, draw=GnBu-M!80!black, scale=0.65},
    draw opacity=0.7,
    fill opacity=0.7,
    mark repeat = 2, 
]

\tikzstyle{mu60_err} = [
    fill=GnBu-M!50,
    fill opacity=0.5,
]

